Cactus: Towards Psychological Counseling Conversations using Cognitive Behavioral Theory

Recently, the demand for psychological counseling has significantly increased as more individuals express concerns about their mental health. This surge has accelerated efforts to improve the accessibility of counseling by using large language models (LLMs) as counselors. To ensure client privacy, training open-source LLMs faces a key challenge: the absence of realistic counseling datasets. To address this, we introduce Cactus, a multi-turn dialogue dataset that emulates real-life interactions using the goal-oriented and structured approach of Cognitive Behavioral Therapy (CBT). We create a diverse and realistic dataset by designing clients with varied, specific personas, and having counselors systematically apply CBT techniques in their interactions. To assess the quality of our data, we benchmark against established psychological criteria used to evaluate real counseling sessions, ensuring alignment with expert evaluations. Experimental results demonstrate that Camel, a model trained with Cactus, outperforms other models in counseling skills, highlighting its effectiveness and potential as a counseling agent. We make our data, model, and code publicly available.

==> figures/app_camel_bad_case.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{images/app_camel_bad.png}
    \caption{Example of the limitation of \textsc{Camel-LLaMA3}.}
    \label{fig:app_camel_bad}
\end{figure*}

==> figures/data_distribution_figure.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/sample_data_distribution.png}
    \caption{The distribution of CACTUS dataset}
    \label{fig:distribution}
\end{figure}

==> figures/method_figure.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{images/method.png}
    \caption{Data collection pipeline for \ourdatas{}.}
    \caption{Data collection pipeline for \ourdatas{}.}
    \label{fig:overall_pipeline}
\end{figure*}

==> tables/ab_exp_2.tex <==
\begin{table*}[!ht]
\centering
\resizebox{0.8\textwidth}{!}
{
\begin{tabular}{lcccc}
    \toprule
    \multirow{2.5}{*}{Model} & \multicolumn{4}{c}{General Counseling}  \\ 
    \cmidrule(lr){2-5}
  & Agenda Setting  & Understanding & Interpersonal Eff. & Collaboration    \\
    \midrule    
    \textsc{Camel-llama3} & . & . & . & .  \\
      ~ w/o diverse attitude & . & . & . & . \\ 
      ~ w/o filtering & 2.28 & 4.01 & 5.04 & 3.64 \\ 
    \bottomrule
\end{tabular}
}
\caption{Ablation Study to demonstrate effectiveness of our steps (It will be a figure), w/o diverse attitude means only positive attitude.}
\label{tab:ablation_method}
\end{table*}

==> tables/app_correlation.tex <==
\begin{table*}[!t]
\centering
% \small
\resizebox{0.98\linewidth}{!}
{
\begin{tabular}{lcccc}
    \toprule
    \multirow{2.5}{*}{Evaluator} & \multicolumn{2}{c}{General Counseling}  & \multicolumn{2}{c}{CBT-specific} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & pairwise & score & pairwise & score \\
    \midrule
    Human & 0.12 & 0.55 & 0.38 & -0.06 \\
    GPT-4o & \textbf{0.30} & \textbf{0.66} & \textbf{0.76} & \textbf{0.61} \\
    \bottomrule
\end{tabular}
}

\caption{Accuracy for Pearson correlations between expert and other evaluator.}
\label{tab:correlation}
\end{table*}

==> tables/cbt-llm_exp.tex <==
\begin{table*}[t!]
\centering
\resizebox{0.9\textwidth}{!}
{
\begin{tabular}{lcccccccc}
    \toprule
    \multirow{2.5}{*}{Model}  & \multicolumn{3}{c}{General Counseling Skills} & \multicolumn{3}{c}{CBT-specific Skills}  \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    & Understanding & Interpersonal Eff. & Collaboration & Guided Discovery  & Focus & Strategy \\
    \midrule
    CBT-LLM  & 4 & 5.12 & 3.79 & 2.66 & 3.95 & 4.02 \\
    \midrule
    \textbf{\textsc{Camel-llama2}} & \textbf{4.20} & \textbf{5.41} & \textbf{4.42} & \textbf{3.80} & \textbf{4.07} & \textbf{4.81} \\
    \textbf{\textsc{Camel-llama3}} & \textbf{4.42} & \textbf{5.97} & \textbf{4.81} & \textbf{4.40} & \textbf{4.11} & \textbf{5.11} \\
    \bottomrule
\end{tabular}
}
\caption{Results of \textsc{CounselingEval} on general counseling and CBT-specific skills for the trained models.}
\label{tab:cbt-llm_exp}
\end{table*}

==> tables/dialogue_sample.tex <==
\begin{table}
\centering
\small
\begin{tabular}{p{7cm}} 
\toprule
\textbf{Thought}: I have been a straight A student for 11 years, but I got one B today. I'll never be an astronaut now.

\textbf{Cognitive distortion}: Catastrophizing, Discounting the Positive \\
\midrule
\textbf{Intake form}

\textbf{Reason for Seeking Therapy}

The client is seeking therapy due to experiencing intense emotional distress and self-doubt after receiving a grade lower than expected. They fear that this single setback will have a permanent impact on their future aspirations and are struggling with anxiety related to this event.

\textbf{Cognitive Distortions Observed}

Catastrophizing: The client tends to magnify the consequences of a minor setback, believing it will lead to disastrous outcomes.

Discounting the Positive: Despite a long history of academic success, the client minimizes their achievements and focuses on the negative aspects. \\
\midrule
\textbf{Dialogue}

\textbf{Counselor}: Welcome to our first session. I'm glad you reached out for support. Let's start by talking about what brought you here today. What's been going on that made you decide to seek therapy?

\textbf{Patient}: I received a grade lower than I expected on an important assignment, and it has really shaken my confidence. I feel like this one setback is going to ruin everything for me.

\textbf{Counselor}: It sounds like this experience has been really distressing for you. Let's explore some of the thoughts and feelings you've been having since then. Have you noticed any patterns in the way you've been thinking about this situation?

\textbf{Patient}: I keep thinking that this one grade is going to determine my entire future. I can't stop imagining all the negative consequences of this setback.

\textbf{Counselor}: It sounds like you might be catastrophizing this situation, imagining the worst possible outcomes. Let's work on challenging these catastrophic thoughts. Can you think of any other perspectives that might offer a more balanced view of the situation?

\textbf{Patient}: I guess I've had other successes in the past that shouldn't be discounted because of this one setback.

:

:

:
 \\
\bottomrule 
\end{tabular}
\caption{A sample dialogue of CACTUS.}
\label{tab:patient_questions}
\end{table}

==> tables/downstream_performance_auto.tex <==
\begin{figure*}[htbp]
    \centering
    \small
    
    \begin{subfigure}[b]{\textwidth}
        \centering
        \small 
        
        \begin{tabular}{clrrrrrr}
            \toprule
            %&& \multicolumn{6}{c}{Eval Dataset}  \\
            \multirow{2.5}{*}{Model}          & \multirow{2.5}{*}{Training Data}  & \multicolumn{2}{c}{Psych8k} & \multicolumn{2}{c}{SMILECHAT} & \multicolumn{2}{c}{\ourdatas{}}  \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
                                            &                      & BLEU & BERT Score & BLEU & BERT Score   & BLEU & BERT Score  \\
                                            \midrule
            ChatGPT                          & ---                  & 7.14 & 13.44 & 2.22 & 6.96 & 20.3 & 38.1 \\
            GPT-4                         & ---                  & 5.42 & 10.61 & 1.65 & 5.41 & 23.8 & 41.3 \\ \midrule
            \multirow{4}{*}{Llama 2 7B}
            % & Oracle               & 0.28 & 4.18 & 0.12 & 1.66 & 8.0 & 37.2 \\ \cmidrule{2-8}
            & Psych8k               & \textbf{4.20} & 8.45 & \textbf{1.55} & 4.80 & 20.3 & 41.3 \\
                                            & SMILECHAT          & 40.51 & 8.77 & 9.36 & 7.85 & \textbf{28.3} & \textbf{57.7} \\
                                            & CBT-LLM & 6.28 & \textbf{8.37} & 1.70 & \textbf{4.66} & 28.3 & 57.2 \\ 
                                            & \ourdatas{} & 6.28 & \textbf{8.37} & 1.70 & \textbf{4.66} & 28.3 & 57.2 \\ \midrule
                                            % & Both & 6.28 & \textbf{8.37} & 1.70 & \textbf{4.66} & 28.3 & 57.2 \\ \midrule
            \multirow{3}{*}{Llama 3 8B}     & Psych8k               & 3.75 & 8.40 & 0.97 & 4.22 & 21.2 & 41.0 \\
                                            & SMILECHAT          & 38.48 & 8.99 & 32.10 & 5.70 & \textbf{33.1} & \textbf{57.8} \\
                                            & \ourdatas{} & \textbf{3.58} & \textbf{8.15} & \textbf{0.97} & \textbf{4.19} & 31.8 & 57.8 \\
            \bottomrule
        \end{tabular}
        \vspace{0.5cm}
    \end{subfigure}
    \hfill
    
\caption{Fact Duration Prediction Results. On the left, we report our full results, with performance split by model type and training data. Performance on SituatedQA and TimeQA are given as the mean average error in years (Y) and mean squared error in years in log-seconds (LS), the same as the regression system training loss. On the right, we depict error histograms evaluated on SituatedQA, with systems trained on TimeQA.}
\label{fig:fact_duration_results_hist}
\end{figure*}

==> tables/main_exp_1.tex <==
\begin{table}[htbp]
\centering
\small
\resizebox{0.96\linewidth}{!}
{
\begin{tabular}{lcccccccc}
    \toprule
    \multirow{4}{*}{LLaMA3-8B}      
    & SMILECHAT     & 8.77 & 9.36 & 7.85 & 1.70  \\
    & \textsc{Cactus}-ch & 6.28 & \textbf{8.37} & 1.70 & 1.70 \\ 
    \cmidrule(lr){2-6}
    & Psych8k  & \textbf{8.37} & 1.70 & \textbf{4.66} & 1.70  \\
    & \textsc{Cactus} & 6.28 & \textbf{8.37} & 1.70 & 1.70 \\ 
    \bottomrule
\end{tabular}
}
\caption{The evaluation of the general counseling skills of the model fine-tuned with multiple datasets.}
\label{fig:main_exp_1}
\end{table}
